An Empirical Analysis of Privacy in the Lightning Network

Payment channel networks, and the Lightning Network in particular, seem to offer a solution to the lack of scalability and privacy offered by Bitcoin and other blockchain-based cryptocurrencies. Previous research has focused on the scalability, availability, and crypto-economics of the Lightning Network, but relatively little attention has been paid to exploring the level of privacy it achieves in practice. This paper presents a thorough analysis of the privacy offered by the Lightning Network, by presenting several attacks that exploit publicly available information about the network in order to learn information that is designed to be kept secret, such as how many coins a node has available or who the sender and recipient are in a payment routed through the network.

==> Makefile <==
.PHONY : main

MAIN=ln_paper
LATEX=pdflatex 

all: paper tidy

paper: $(MAIN).tex
	$(LATEX) -synctex=1 -interaction=nonstopmode $(MAIN).tex
	bibtex $(MAIN).aux
	$(LATEX) -synctex=1 -interaction=nonstopmode $(MAIN).tex
	$(LATEX) -synctex=1 -interaction=nonstopmode $(MAIN).tex
	bibtex $(MAIN).aux
	$(LATEX) -synctex=1 -interaction=nonstopmode $(MAIN).tex

no_comments:
	pdflatex "\AtBeginDocument{\input{disable_comments.sty}}\input{ln_paper.tex}"
	bibtex $(MAIN)
	pdflatex "\AtBeginDocument{\input{disable_comments.sty}}\input{ln_paper.tex}"
	pdflatex "\AtBeginDocument{\input{disable_comments.sty}}\input{ln_paper.tex}"
	bibtex $(MAIN)
	pdflatex "\AtBeginDocument{\input{disable_comments.sty}}\input{ln_paper.tex}"

tidy:
	rm -f *.dvi *.aux *.log *.nav *.snm *.toc *.out *.vrb *.blg *.synctex.gz *.ps

clean:
	rm -f *.dvi *.aux *.log *.nav *.snm *.toc *.out *.vrb *.blg *.synctex.gz $(MAIN).ps $(MAIN).pdf

